Scaling Mesh Generation via Compressive Tokenization

We propose a compressive yet effective mesh representation, Blocked and Patchified Tokenization (BPT), facilitating the generation of meshes exceeding 8k faces. BPT compresses mesh sequences by employing block-wise indexing and patch aggregation, reducing their length by approximately 75\% compared to the original sequences. This compression milestone unlocks the potential to utilize mesh data with significantly more faces, thereby enhancing detail richness and improving generation robustness. Empowered with the BPT, we have built a foundation mesh generative model training on scaled mesh data to support flexible control for point clouds and images. Our model demonstrates the capability to generate meshes with intricate details and accurate topology, achieving SoTA performance on mesh generation and reaching the level for direct product usage.

==> sec/XX_intro.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/data3.png}
\caption{\textbf{Scaling mesh generation with data containing more faces.} (a) BPT can handle meshes with up to 8k faces, showing the potential to utilize vast amounts of high-quality mesh data
with rich details. (b) As the complexity of the mesh data
increases, the performance and generalizability of the model are significantly improved.
}
\label{fig: data}
\end{figure*}


\section{Introduction}


% #### Background

Meshes, serving as the cornerstone of 3D geometric representation, are widely utilized across a spectrum of applications, including video games, cinematic productions, and architectural modeling.
Despite their widespread adoption, the meticulous craft of meshes with functional topologies demands substantial design effort. This labor-intensive process acts as a bottleneck, impeding both the evolution of 3D content creation and the progress of immersive human-computer interaction.
Recent researches \cite{siddiqui2023meshgpt,chen2024meshxl,weng2024pivotmesh,chen2024meshanything,chen2024meshanythingv2,tang2024edgerunner} try to automate the mesh sculpting process via auto-regressive Transformers.
These methods directly generate vertices and faces as human-crafted to maintain the high-quality mesh typology, yielding promising performance on low-poly generation.

% Q: Why do these methods fail to generate high-quality polygon mesh?
% A: Cannot access training data with many faces;
% Q: Why do these methods cannot access training data with many faces?
% A: Redundant representations;
% Q: Why are the representations redundant?
% A: 1. Inefficient vertex tokenization;
%    2. Redundant face tokenization;

% Challenges in Existing Mesh Generation Methods
% It is unclear why they cannot train on high-poly mesh.
Despite the efficacy of current mesh generative models, they often fall short in producing meshes with intricate topologies. This limitation is primarily attributed to their training datasets, which predominantly consist of low-poly meshes, leading to inadequate generalization capabilities for generating fine details.
Recent efforts focus on leveraging more compact mesh representations to extend the scope of training data within the limited Transformer context window.
Some methods \cite{siddiqui2023meshgpt,weng2024pivotmesh,chen2024meshanything} utilize auto-encoder to compress meshes into latent sequences, albeit at the expense of reconstruction quality.
On the other hand, MeshAnythingv2 \cite{chen2024meshanythingv2} and Edgerunner \cite{tang2024edgerunner} propose novel tokenization methods to reduce the length of vanilla mesh sequences. 
However, the representation of these approaches is still redundant, constrained to handling meshes with at most 4k faces.
As shown in Figure \ref{fig: data}(a), meshes within 4k faces contain some delicate structures but still lack details.
\textit{To scale up mesh generation, a more compressive mesh representation is required to extend the training data scope.}

% Scale-up mesh generation is more like the result of BPT.
% Q: How do we scale up mesh generation?
% A: A compressive representation is required;
% Q: How can we do that?
% A: 1. Compress vertex tokenization (Block indexing);
%    2. Compress face tokenization (Patch aggregation);
% proposed method
In this paper, our primary goal is to scale up mesh generation with data containing more faces (i.e., with more details).
We propose a compressive yet efficient mesh representation called Blocked and Patchified Tokenization (BPT).
BPT first converts Cartesian coordinates to block-wise indexing, then aggregates all the faces connected with the selected center vertices as patches.
Our approach significantly reduces the length of the vanilla mesh sequence with around 75\% compression.
As shown in Figure \ref{fig: data}(a), BPT can handle meshes with up to 8k faces, showing the potential to utilize vast amounts of high-quality mesh data with rich details.
Furthermore, we make the initial step to show the boosted performance afforded by the scaled data with more faces.
Figure \ref{fig: data}(b) illustrates the positive correlation between the number of faces and the performance of generative models: as the complexity of the mesh data increases, the performance and generalizability of the generative models are significantly improved.

% Applications and Results

BPT facilitates a wide range of 3D applications. We demonstrate its effectiveness via conditional mesh generation on point clouds and images with the auto-regressive Transformer.
Our model empowers even unprofessional users to produce meshes at the product-ready level within several minutes.
The applicability of our model spans a spectrum of practical domains, including video gaming, product design, and the creation of immersive experiences, revealing the dawn of a new era in 3D generation.

% 1. BPT achieves a high compress ratio;
% 2. Leveraged with BPT, we build the first mesh generative model that could directly train and infer with 8K faces;
% 3. The huge influence.
% Contributions
Our contributions can be summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We introduce Blocked and Patchified Tokenization (BPT), a compressive yet efficient tokenization with a state-of-the-art compression ratio of around 75\%.
   \item We make an initial step towards scaling mesh generation on data with more faces, and reveal that the generation performance and generalizability are significantly boosted with the scaled data.
    \item We build a mesh foundation model that supports conditional generation based on both images and point clouds, enabling even non-professional users to create product-ready 3D assets.
\end{itemize}



